Quda: Natural Language Queries for Visual Data Analytics

The identification of analytic tasks from free text is critical for visualization-oriented natural language interfaces (V-NLIs) to suggest effective visualizations. However, it is challenging due to the ambiguity and complexity nature of human language. To address this challenge, we present a new dataset, called Quda, that aims to help V-NLIs recognize analytic tasks from free-form natural language by training and evaluating cutting-edge multi-label classification models. Our dataset contains $14,035$ diverse user queries, and each is annotated with one or multiple analytic tasks. We achieve this goal by first gathering seed queries with data analysts and then employing extensive crowd force for paraphrase generation and validation. We demonstrate the usefulness of Quda through three applications. This work is the first attempt to construct a large-scale corpus for recognizing analytic tasks. With the release of Quda, we hope it will boost the research and development of V-NLIs in data analysis and visualization.

==> src/__latexindent_temp.tex <==
\section{\name{} Applications}

\name{} benefits the construction of V-NLIs by training and benchmarking state-of-the-art neural networks.
% , based on which V-NLIs are able to identify analytic tasks for free-form natural language.
The first case demonstrates the characteristics of \name{} by training and benchmarking a well-performing multi-label classification model. 
We then present an example to showcase how \name{} can improve an existing NLI toolkit in task inference.
Finally, we explore how \name{} can assist intelligent hinting in a V-NLI interface.

\subsection{Multi-label Text Classification}
\label{subsec:multilabel}
Assigning all task labels to a query is critical to V-NLIs.
Therefore, we conduct an experiment to evaluate how a well-performed multi-label classification models perform on our corpus, and reveal the characteristics of our corpus with different experiment settings.

\subsubsection{Model}
Recent research in pre-trained models~\cite{Devlin2019,Yang2019} has achieved state-of-the-art performance in many of the NLP tasks.
These models are trained on large corpus, \eg, all wikipedia articles, and allow us to fine-tune them on downstream NLP tasks, such as multi-label text classification.
Here, we conduct our experiment with a well-known pre-trained model, Bert, which obtained new state-of-the-art results on eleven NLP tasks when it was proposed~\cite{Devlin2019}.
We trained the two models for $3$ epochs, and use a batch size of $2$ and sequence length as $41$, \ie, the maximum possible in our corpus. 
The learning rate was set as $3e-5$, the same as in the original paper.

\subsubsection{Dataset and Evaluation Metrics}
Different data splits (train and test) may affect the performance of models. 
We split \name{} in two ways. First, we randomly split it into train ($11228$ samples) and test ($2807$ samples), and name it as \name{}\_random.
Second, we split the dataset by experts (\name{}\_expert). 
That is, 20 experts are split into train ($16$ experts) and test sets ($4$ experts), and all queries created by the same experts and their paraphrases are in the same set.
We obtain $11065$ samples for training and $2970$ samples for test.
Following the work~\cite{Wang2016}, we employ precision and recall as evaluation metrics.
% The definitions are presented in Equation~\ref{eq:precision} and~\ref{eq:recall}, respectively.  
% \begin{equation}
%     \label{eq:precision}
% \mathbf{Precision}=\frac{\textrm{The number of correctly annotated labels}}{\textrm{The number of predicted labels}}
% \end{equation}
% \begin{equation}
%     \label{eq:recall}
% \mathbf{Recall}=\frac{\textrm{The number of correctly annotated labels}}{\textrm{The number of ground-truth labels}}
% \end{equation}

% Besides \name{}, we have prepared \name{}\_aug in this experiment.
% We observed that high-frequency words that appeared in the \name{} queries may have strong correlations with the contents in the data tables, that is, these words or phrases are values in data tables or synonyms of column names.  
% These correlations may introduce biases and make the model ignoring the real intentions of the queries, and therefore hurting the model generalization.
% Inspired by prior work \cite{Zhang2015}, we further employ a data augmentation technique on \name{} that replaces words or phrases with their synonyms.
% To be specific, we derive a list of $210$ high-frequent words after stop-words removal. 
% Then we manually categorize these words into five groups, \ie, Place, Person, Time, Date, and Others.
% Finally, for each group, we compile a set of alternative words from WordNet\cite{Fellbaum2000}, and replace high-frequent words with the alternatives randomly.
% We split both \name{} and \name{}\_aug randomly into train ($80\%$) and test set ($20\%$). 
% All queries in \name{} and \name{}\_aug are labeled with one or some of the $10$ analytic tasks~\cite{Saket2019}. 

\subsubsection{Results}
The precision and recall of the model on \name{}\_random are $97.7\%$ and $96.0\%$, respectively.
On the other hand, the model performance trained on \name{}\_expert only achieves $84.2\%$ (precision) and $74.3\%$ (recall).
Since the train and test samples of \name{}\_expert are crafted based on different data tables and experts, the syntax space 
may be different. 
As a result, \name{}\_expert is more challenging. 
And this leaves room for developing new methods that specifically designed for this task. 
Though models trained on \name{}\_random have performs better, the performance on \name{}\_expert is close to real-world scenarios since the data tables and users may vary.

To understand how the model on \name{}\_expert performs across different analytic tasks, we investigate the per-class precision and recall.
As shown in Table~\ref{tab:perclass}, the model performs well on tasks such as \textit{Find Extremum}, \textit{Sort}, and \textit{Cluster}.
However, it performs poorly in tasks including \textit{Filter} and \textit{Characterize Distribution}.
In some tasks, such as \textit{Compute Derived Value} (precision: 0.82, recall: 0.51) and \textit{Retrieve Value} (precision: 0.92, recall: 0.64), the model is high in precision while low in recall.
This means the model returns fewer results compared to the ground-truth labels, but most of the predicted labels are correct.
The reason why the model performs well in some tasks but poorly in others remains unknown. 
We leave the problem as future research which involves a deep understanding of the model as well as syntax space of different tasks.




% Figure~\ref{fig:classify_result} shows the performance of two models on \name{} and \name{}\_aug in terms of Hamming Loss, average accuracy, and F1 score. 
% and observe that the precision achieves $97.7\%$ while the recall is about $96\%$.
% Compare to the SOTA precision of the other datasets for text classification at a similar scale (e.g., TREC-$98.07\%$\cite{Cer2018}), the numbers in Figure~\ref{fig:classify_result} indicate that classifying the \name{} queries is challenging, and this leaves room for developing new methods that specifically designed for this task. 
% As shown in Figure~\ref{fig:classify_result}, on average, 
% the augmented corpus (i.e., \name{}\_aug\_expert) increases the precision for about $3.14\%$. This proves that the data augmentation we introduced in this paper is useful for model generalization.

\begin{table}
    \centering
    \begin{tabular}{l|cc}
    \toprule
    \textbf{Task}             & \textbf{Precision} & \textbf{Recall} \\\midrule
    Retrieve Value            & 0.92      & 0.64   \\
    Filter                    & 0.79      & 0.79   \\
    Compute Derived Value     & 0.82      & 0.51   \\
    Find Extremum             & 0.86      & 0.88   \\
    Sort                      & 0.94      & 0.81   \\
    Determine Range           & 0.9       & 0.7    \\
    Characterize Distribution & 0.73      & 0.69   \\
    Find Anomalies            & 0.82      & 0.75   \\
    Cluster                   & 0.88      & 0.91   \\
    Correlate                 & 0.9       & 0.76   \\
    \bottomrule
    \end{tabular}
    \caption{The per-class precision and recall of Bert on \name{}\_expert.}
    \label{tab:perclass}
\end{table}

\subsection{Improving an Existing V-NLI Toolkit}
The multi-label classification model trained with \name{} can benefit existing NLI toolkits in task inference for free-form natural language.
We choose NL4DV~\cite{Narechania2020} as an example, which is the first python-based library that supports prototyping V-NLIs.
NL4DV takes NL queries and a dataset as input, and returns an ordered list of Vega-Lite specifications to respond these queries.
Its query interpretation pipeline includes four modules, such as query parsing, attribute inference, task inference, and visualization generation.
The task inference module of NL4DV focuses on the detection of 1) task type, 2) the parameters associated to a task, and 3) ambiguities of operators and values.
Currently, the toolkit supports five base tasks (\ie, \textit{Correlation}, \textit{Distribution}, \textit{Derived Value}, \textit{Trend}, \textit{Find Extremum}), and \textit{Filter}.
To infer tasks, the authors setup a set of rules according to task keywords, POS tags, dependency tree, and data values.
Although effective in some scenarios, the rule-based approach is hard to extend and limited for free-form natural language.

We aim to improve the precision and range of task type inference with the help of \name{}.
We first use Bert\cite{Devlin2019} trained on \name{}\_expert (details are introduced in Section~\ref{subsec:multilabel}) for the detection of task type.
Our model supports ten low-level tasks and can assign multiple tasks labels for each query. 
Though our model cannot explicitly detect the \textit{Trend} task supported by NL4DV, \textit{Trend} is usually identified as \textit{Correlation} and \textit{Distribution}, and appropriate visualizations are recommended.
For example, \textit{``Illustrate the distribution of the population of Ashley across the five years.''} is identified as \textit{Correlation} and \textit{Filter}. 
Second, we setup a set of rules to generate visualization for all tasks.
Similar to NL4DV, the ten tasks are divided into $9$ base tasks and \textit{Filter}.
For base tasks, we take into account the type of data attributes and tasks to identify proper visualizations and visual encodings.
For \textit{Filter} and its associated attributes, we highlight information in the Bar chart rather than filter to few bars according to the design guideline~\cite{Hearst2019}.

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{pictures/nl4dv.pdf}
    \caption{Four examples showcase that NL4DV\_\name{} can improve NL4DV in identifying tasks with higher precision  (a and b) and supporting more analytic tasks (c and d).}
    \label{fig:nl4dv}
\end{figure}


% To demonstrate how \name{} benefits the NL4DV library, we show corner cases where NL4DV fails
\subsubsection{Case Study}
We demonstrate that \name{} can improve the robustness of NL4DV in task inference.
We compare the results generated by NL4DV and the augmented library (named NL4DV\_\name{}) using a movie dataset.
Admittedly, NL4DV is able to generate reasonable visualizations in most cases. 
However, it fails when tasks are not correctly detected.
In the first example, we demonstrate that incorrect task inference leads to ineffective visualizations. 
Figure~\ref{fig:nl4dv}(a) shows the results of \textit{``How does the budget distribute across different genres?''}
NL4DV identifies the sentence as \textit{Derived Value} according to the type of attributes, and calculates mean budget for each genre.
However, the mean budget cannot characterizes budget distribution for each genre.
NL4DV fails to detect the query as \textit{Distribution} because ``distribute'' is not included in the task keywords.
NL4DV\_\name{}, on the other hand, detect the task as \textit{Distribution} and respond the query using a strip plot.
We observe that the budget of action movies distribute evenly between 20 millions and 150 millions.
While most comedy movies have budget around 20 millions.

The second example shows that NL4DV may miss tasks associated with a query. 
The query, \textit{``How many Drama movies are there in this table?''} belongs to \textit{Derived Value} and \textit{Filter} because drama movies should be filtered from all genres and the amount is derived through a count operator.
The attribute inference module of NL4DV detects one data value (drama) only.
Hence, NL4DV merely identifies it as \textit{Filter} and shows a bar chart with severe visual clutter (Figure~\ref{fig:nl4dv}(b)).
On the other hand, NL4DV\_\name{} correctly recognizes both tasks. 
It show a bar chart with count operator to respond the \textit{Derived Value} task, and further highlights drama movies to \textit{Filter}.


% NL4DV detects it as \textit{Filter}. 
% The histogram presented by NL4DV helps little in the identification of the longest running time.
% On the other hand, NL4DV\_\name{} recognizes the query as \textit{Find Extremum} and displays a boxplot to show statistical distribution of running time for all movies. 
% When hovering over the boxplot, a tooltip is displayed showing that the max running time is $194$.

% Figure~\ref{fig:nl4dv}(a) shows the results of \textit{``How many Drama movies are there in this table?''}
% This sentence belongs to \textit{Derived Value} and \textit{Filter} because the number of Drama movies should be derived through a count operator for the Genre attribute.
% Both \textit{Derived Value} and \textit{Filter} are common tasks of NL4DV and NL4DV\_\name{}.
% However, NL4DV merely identifies it as \textit{Filter} and shows a bar chart with severe visual clutter.
% fails to detect the \textit{Derived Value} task and shows a bar chart with severe visual clutter.
% On the other hand, NL4DV\_\name{} can recognize \textit{Derived Value} and count the number of records for each Genre.
% Further, 

Thirdly, we illustrate that NL4DV\_\name{} supports a broader range of analytic tasks compared to NL4DV, including \textit{Determine Range}, \textit{Retrieve Value}, \textit{Sort}, and \textit{Find Anomalies}. 
% By default, NL4DV infers analytic tasks according to the type of data attributes and task keywords.
% In some cases, incorrect task inference may result ineffective visualizations.
Taking the query \textit{``what is the range of budget''} as an example, NL4DV detects it as \textit{Distribution} based on the type of data attribute, and shows a histogram for production budget (Figure~\ref{fig:nl4dv}(c)).
However, the binning operation hinders users from identifying the minimum and maximum value.
Similarly, NL4DV detects the query, \textit{``Are there any outliers in the budget''}, as distribution and depicts a histogram by default (Figure~\ref{fig:nl4dv}(d)).
The histogram, however, fails to reveal movies with abnormal budget.
NL4DV\_\name{} can correctly detect the tasks and present an appropriate visualization in each case.
As shown in Figure~\ref{fig:nl4dv}(c) and (d), NL4DV\_\name{} shows boxplots with different parameter settings to demonstrate the range and outliers, respectively.

% To conclude, the above two examples show cases where NL4DV may fail due to the defects in task inference.
% Compared with the rule-based technique provided by NL4DV, 
To conclude, due to the defects in task inference, NL4DV may result in ineffective visualizations.
The model trained on \name{}, on the other hand, is more robust in multi-label task classification.
Further, the model supports more analytic tasks which extends NL4DV to a wider range of usage scenarios. 

\subsection{Query Recommendation for V-NLIs}
Some V-NLIs, such as Eviza~\cite{Setlur2016}, Articulate~\cite{Sun2010}, and FlowSense~\cite{Yu2020}, have embedded template-based auto-completion to improve user experience~\cite{Gao2015}.
That is, after a user query is partially completed, the interface provides hints for possible queries.
Though useful, these techniques are tailored to specific applications and grammars, and can hardly be generalized to other V-NLIs.
Query recommendation techniques in search engine~\cite{BaezaYates2005,Zhang2006,Anagnostopoulos2010} suggest a list of related queries based on previously issued queries, which are independent of applications and have wide usage scenarios.
With the help of \name{}, we aim to develop a query recommendation technique for V-NLIs, which recommends semantically meaningful queries based on user input, data table, and \name{}.

\subsubsection{Technique Overview}
We first present the data annotation step that adapts \name{} to our query recommendation technique.
Then, we introduce our technique comprised of three modules: (1) \textit{candidate generation}, (2) \textit{candidate refinement}, and (3) \textit{interactive interface}.

In data annotation, we manually label $920$ expert-generated queries for demonstration, and plan to annotate all $14,035$ queries in \name{} in future research.
For each query, we distinguish phrases or words that are data attributes and data values. 
We further annotate the type of attribute as quantitative, nominal, ordinal, and temporal.
For example, given a query \textit{``what is the \dattribute{birth} distribution of the different \dattribute{districts} in \dvalue{2017}''}, we annotate ``birth'' as data attribute with type quantitative, ``districts'' as data attributes with type nominal, and ``2017'' with type temporal.

The three modules of our technique interacts with each other.
Given a user input, the goal of the \textit{candidate generation} module is to identify candidate queries among $920$ queries that are semantically equivalent to the input.
We borrow universal sentence encoder~\cite{Cer2018} to vectorize $920$ queries and the user input. 
Then, we use Euclidean distance to rank and filter top $5$ candidate queries that are semantically ``close'' to the user input, which result in a set of queries.
Since candidate queries do not relate to the data table, the recommendation, however, may not be meaningful for users.
The \textit{candidate refinement} module aims to refine the candidate queries by replacing data attributes (or values) in candidate queries with those in data table.
We setup two criteria in the replacement: 1) the type of data attributes (or values) should be the same, and 2) the semantics should be as similar as possible.
Finally, we borrow NL-driven Vega-Lite editor~\cite{Narechania2020} as a test bed to showcase our query recommendation technique.
The interface is a Vega-Lite editor~\cite{Satyanarayan2017} enhanced with NL4DV which is a python-based NLI toolkit, which consists of a input bar, an editor for Vega-Lite specification, a panel for visualization results, and a panel for design alternatives.
When a user stops typing in the input bar, the input text is sent to the \textit{candidate generation} module.
After candidate queries are tuned by the \textit{candidate refinement} module, the results are shown in a dropdown menu.

\subsubsection{Usage Scenario}

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{pictures/recommend.pdf}
    \caption{Given a data table (a), our technique recommends queries for three user inputs (b, c, d).}
    \label{fig:recommend}
\end{figure}

Suppose Jane is a fan of Hollywood movies, and she exhibits considerable interest in analyzing a movie dataset containing $709$ records with $10$ fields, including Running Time, Title, Genre, etc (Figure~\ref{fig:recommend}(a)). 
After selecting the Movies dataset, Jane want to see how IMDB ratings are distributed. 
Then she types \textit{``what is the distribution''}.
A dropdown menu is then displayed showing the top $5$ queries recommended by our technique (Figure~\ref{fig:recommend}(b)).
The recommendation accelerates the input process, and Jane simply selects the third query for investigation.
Next, Jane wants to find abnormal movies in the dataset.
However, she has no idea where to start because there are  multiple ways to define whether a movie is abnormal.
She types \textit{``any outlier''} and pauses.
Our technique returns five queries to inspire her with possible definition (Figure~\ref{fig:recommend}(c)).
The first sentence catches her eye.
IMDB rating is a commonly-used criterion to evaluate the quality of a movie.
She chooses the first sentence for detailed inspection.
Finally, Jane wonders whether there are correlations between any data attributes, and types \textit{``correlation''}'.
The dropdown menu shows five possible results (Figure~\ref{fig:recommend}(d)).
Two of them suggest the correlation between release year and production budget.
Hence, Jane decides to start with the first query.
Finally, she concludes, \textit{``The query recommendation not only accelerates my exploration process, but also give me valuable suggestions when I do not exactly know what to see.''}




% \subsubsection{Query Annotation.}
% Our technique relies on the annotation of data attributes and data values.
% % To suggest semantically meaningful queries, we further annotate queries from two aspects.
% % Before 
% We annotate  $920$ expert-generated queries for demonstration.
% To be specific, we manually annotate noun phrases 

% \subsubsection{Architecture of Query Recommendation.}

% The data preprocessing module 

% To suggest candidates that reflect
% \name{} contains $14,035$ human-generated queries.



% Figure~\ref{fig:interface} illustrate the pipeline for our query recommendation technique.
% First, we 





==> src/application.tex <==
\section{\name{} Applications}

\name{} benefits the construction of V-NLIs by training and benchmarking a multi-label classification model, based on which V-NLIs are able to identify analytic tasks for free-form natural language.
The first case demonstrates the characteristics of \name{} by benchmarking of a set of learning-based approaches. 
We then explore the use of \name{} in bootstrapping a V-NLI and augmenting an existing NLI toolkit.
% the analysis of design tasks in academic literature in two domains.

\subsection{Multi-label Text Classification}
Assigning all task labels to a query is critical to V-NLIs.
Therefore, we conduct an experiment to evaluate how a well-performed multi-label classification models perform on our corpus, and reveal the characteristics of our corpus with different experiment settings.

\textbf{Models:}
Recent research in pre-trained models~\cite{Devlin2019,Yang2019} has achieved state-of-the-art performance in many of the NLP tasks.
These models are trained on large corpus, \eg, all wikipedia articles, and allow us to fine-tune them on downstream NLP tasks, such as multi-label text classification.
Here, we conduct our experiment with a well-known pre-trained model, Bert, which obtained new state-of-the-art results on eleven NLP tasks when it was proposed~\cite{Devlin2019}.
We trained the two models for $3$ epochs, and use a batch size of $2$ and sequence length as $41$, \ie, the maximum possible in our corpus. 
The learning rate was set as $3e-5$, the same as in the original paper.

\textbf{Dataset:}
% Besides \name{}, we have prepared \name{}\_aug in this experiment.
% We observed that high-frequency words that appeared in the \name{} queries may have strong correlations with the contents in the data tables, that is, these words or phrases are values in data tables or synonyms of column names.  
% These correlations may introduce biases and make the model ignoring the real intentions of the queries, and therefore hurting the model generalization.
% Inspired by prior work \cite{Zhang2015}, we further employ a data augmentation technique on \name{} that replaces words or phrases with their synonyms.
% To be specific, we derive a list of $210$ high-frequent words after stop-words removal. 
% Then we manually categorize these words into five groups, \ie, Place, Person, Time, Date, and Others.
% Finally, for each group, we compile a set of alternative words from WordNet\cite{Fellbaum2000}, and replace high-frequent words with the alternatives randomly.
% We split both \name{} and \name{}\_aug randomly into train ($80\%$) and test set ($20\%$). 
% All queries in \name{} and \name{}\_aug are labeled with one or some of the $10$ analytic tasks~\cite{Saket2019}. 


\textbf{Results:}
Figure~\ref{fig:classify_result} shows the performance of two models on \name{} and \name{}\_aug in terms of Hamming Loss, average accuracy, and F1 score. 
% Compare to the SOTA precision of the other datasets for text classification at a similar scale (e.g., TREC-$98.07\%$\cite{Cer2018}), the numbers in Figure~\ref{fig:classify_result} indicate that classifying the \name{} queries is challenging, and this leaves room for developing new methods that specifically designed for this task. 
% As shown in Figure~\ref{fig:classify_result}, on average, 
the augmented corpus (i.e., \name{}\_aug\_expert) increases the precision for about $3.14\%$. This proves that the data augmentation we introduced in this paper is useful for model generalization.

\begin{table}
    \centering
    \begin{tabular}{llll|lll}
    \toprule
    \multirow{2}{2cm}{Evaluation Criterion} & \multicolumn{3}{c}{\name{}}  & \multicolumn{3}{c}{\name{}\_aug} \\ \cmidrule{2-7}
        & Bert & Roberta & XLNet & Bert & Roberta & XLNet \\ \midrule
        Hamming Loss & 0.008 & 0.008 & 0.008 & 0.017 & 0.017 & 0.019 \\ \midrule
        Accuracy & 0.940 & 0.941 & 0.941 & 0.876 & 0.876 & 0.862 \\ \midrule
        F1 Score & 0.968 & 0.970 & 0.969 & 0.934 & 0.935 & 0.927 \\ 
    \bottomrule
    \end{tabular}
    \caption{The performance of three baseline models on \name{} and \name{}\_aug.}
    \label{tab:para_stat}
\end{table}


\subsection{Building a V-NLI from Scratch}
% This example showcases how \name{} can help bootstrap a V-NLI system.
% Our research is motivated by the rising trend of V-NLI.
With the large design space~\cite{Yu2020}, one challenge faced by V-NLI design is choosing a proper visualization to answer an analytic question, which relies on the recognition of analytic tasks. 
Given the type of task, V-NLIs can make an effective design choice based on a large body of empirical research~\cite{Saket2019}.
In this section, we present how \name{} can help bootstrap a V-NLI system, called FreeNLI, which highlights in two aspects:
(1) It accepts free-form natural language as input, and (2) forms effective design decision by recognizing multiple analytic tasks from the input query. 

\subsubsection{The FreeNLI System}

Figure~\ref{fig:nli} shows the system architecture of FreeNLI consisting of three major components: a language parser that processes NL query, a pool of design rules that identify effective design decisions, and an interface that interacts with data analysts.

\textbf{Language Parser.}
Given an NL query, FreeNLI parses from two aspects. 
First, it applies a well-trained multi-label classification model, \ie, Bert~\cite{Devlin2019} trained on \name{}\_random, to recognize all analytic tasks involved in the query.
Second, the language parser identifies data fields for visualization.
The mapping from NL to data fields is challenging. 
Due to the sheer variety of natural language expressions, data analysts may use an abbreviation or alternative terms to refer to data fields.
For example, a data table on the performance of basketball players may have two columns, \ie, name and score. 
A data analyst may search for, \textit{``which player (name) has the best performance (score)?''}  
The current prototype uses simple string matching to determine which columns are involved in the visualization.
Therefore, users are required to mention column names in the query.
In future research, we plan to employ more advanced techniques to alleviate this restriction.


\begin{figure}[tb]
    \centering
    \includegraphics[width=.7\linewidth]{pictures/nli.pdf}
    \caption{Overview of the system architecture of FreeNLI.}
    \label{fig:nli}
\end{figure}
\textbf{Design Decisions.}
Based on the findings of an empirical study~\cite{Saket2019}, FreeNLI offers effective design decisions according to data fields, field types, and analytic tasks.
To be specific, we derive design decisions from three aspects, \ie, data transformation, design choice, and design ranking.  
First, to accommodate analytic tasks such as \textit{Find Extreme}, \textit{Characterize Distribution}, and \textit{Compute Derived Value}, we employ simple data transformation and aggregation techniques, such as binning, counting, sorting, deriving maximum, minimum, and average on these tasks.
Next, similar to Voyager~\cite{Wongsuphasawat2016}, FreeNLI construct possible visualizations based data types (numerical and nominal), visualization types (scatterplot, bar chart, pie chart, and line chart).
Finally, we rank possible visualizations based on user preference\cite{Saket2019}.

\textbf{Interface.}
Figure~\ref{fig:interface}(a) shows that FreeNLI provides a concise interface for a user to interact with. 
As a start, a user may select or upload a dataset. 
Then, the dataset is shown as a table with which the user is allowed to navigate raw data and raise hypotheses. 
Simple manipulations, such as sorting and filtering, are supported.
The user can then raise queries for the data table.
When a query is submitted, a pop-up window with effective visualizations will be displayed to answer the query.
The user can hover over visual elements to explore detailed information using a tooltip.
Since FreeNLI was for demonstration purposes, we kept the interface simple and provided limited functionality and customization in the current prototype.
We plan to refine and augment FreeNLI iteratively from two directions. 
First, we plan to provide rich configuration for the visualization and data transformation, such as adjusting the size of binning, including pivoting, sampling, etc.
Second, we will improve user experience with more features, such as exploratory analysis and history, etc.

\subsubsection{Usage Scenario}
We describe a usage scenario to evaluate the usefulness of FreeNLI.
Suppose Jane is a fan of Hollywood movies, and she exhibits considerable interest in analyzing a movie dataset comprising nine fields, including budget, title, genre, votes, etc. 
The dataset contains a total of $2,681$ records, and she aims to gain a comprehensive sense of the dataset and identify trends, distribution, or other insights worth sharing.
After loading the movie dataset to FreeNLI, a data table is shown to allow Jane to explore the dataset by sorting and filtering.
\textit{``I do not want to use the table to explore such a large dataset''}, Jane murmurs.
Instead, she decides to ask questions to visualize the dataset.
For an overview of worldwide gross profit, Jane types the query \textit{``How about the worldwide gross profit of different genres?''}.
A bar chart pops up to display the distribution of \textit{Genre} on \textit{Worldwide Gross} profit (Figure~\ref{fig:interface}(b)). 
She observes that adventure movies have the grossest profit compared to other types of movies.
Jane wonders whether adventure movies are released more than others. 
She then asks \textit{``Show me the distribution of genre.''}
FreeNLI shows a pie chart to address this query (Figure~\ref{fig:interface}(d)).
Surprisingly, \textit{Adventure} only accounts for $9.2\%$ among all types of movies.
\textit{Drama}, \textit{Comedy} and \textit{Action} have more market share compared to \textit{Adventure}.
Jane infers that adventure movies are usually high in the budget, and only filming teams with enough resources can afford it.
To verify the hypothesis, she asks \textit{``What is the correlation between Genre and Budget?''}
A bar chart is displayed showing that \textit{Adventure} requires the most budget (71 million dollars on average) among all categories (Figure~\ref{fig:interface}(c)).
Finally, she concludes, \textit{``Though adventure movies have high worldwide gross profit, only limited filming teams with a high budget can afford it.''}



\begin{figure}[tb]
    \centering
    \includegraphics[width=.5\linewidth]{pictures/interface.pdf}
    \caption{(A) The interface of FreeNLI. (B)-(D) Two bar charts and one pie chart are displayed to answer different queries. }
    \label{fig:interface}
\end{figure}



% \subsubsection{Discussions and Future Directions}
% A large body of empirical research has evaluated the effectiveness of various design decisions given analytic tasks and datasets.
% However, data analysts without visualization background may not benefit from these studies.
% FreeNLI recognizes analytic tasks for free-form natural language queries and helps data analysts gain insights into data with effective visual representations.
% However, despite its promise, the current prototype is limited in two aspects.
% First, input queries should articulate which data fields are involved. 
% Although this step is common for many existing V-NLIs, it is not natural for free-form NL queries.
% Hence, we plan to remove this restriction by employing models in text-to-SQL to map NL queries to data fields.
% Second, the current prototype is not scalable because of the need to construct a large number of rule-based design strategies.
% The second issue can be resolved by building end-to-end models that can learn expert behaviors in authoring visualizations, which is a promising research direction. 


\subsection{Improving an Existing V-NLI Toolkit}
The multi-label classification model trained with \name{} can also benefit existing NLI toolkits.
We choose NL4DV as an example, which is a python-based library that supports prototyping V-NLIs.
Specifically, its query interpretation pipeline includes query parsing, attribute inference, task inference, and visualization generation.
With the help of \name{}, NL4DV is able to 1) extend task inference 

% \subsection{Comparison of Two Application Fields}
% To demonstrate the usefulness of our corpus beyond V-NLIs, we analyze and compare the design requirements of two application domains, \ie, visual analytics of sports data and urban computing.
% To answer questions such as, \textit{``How tasks distributed in the two domains''} and \textit{``What are dominant tasks in each domain''}, 
% we first collect $54$ publications from leading venues. 
% Then, we manually gather task utterances from the publications.
% Next, we employ the \textit{Ad-RNN} model trained on \textit{\name{}\_aug\_expert} and classify task utterances into $10$ categories. 
% We include an \textit{``Others''} category to handle utterances that do not belong to any of the $10$ tasks. 
% Finally, we report the analytic results in comparing the two domains.

% \subsubsection{Data Collection}
% To ensure that papers are of high quality, we focus on those published in top venues in visual analytics, transportation, and sports analytics, such as IEEE transactions on visualization and computer graphics, IEEE Transactions on Intelligent Transportation Systems, Proceedings of the CHI conference, etc.
% In addition, to obtain design requirements, we selectively choose papers that 1) target at domain problems and 2) solve domain problems using visual analytics.
% Finally, we have collected $54$ papers where $28$ are in the urban domain and $26$ are in the sports domain.
% The full paper list can be found in the supplementary material.

% The text classification model trained on \name{} may have better performance if the data for prediction are in the same vocabulary and syntax space as training samples. 
% Our corpus features queries that are objectives, concrete in the abstraction level, and low in the composition level.
% Therefore, we focus on task utterances that share similar characteristics as our corpus.
% To gather text as required, we have gone through sections related to design tasks, requirement analysis, system design, and case study, and collect all possible utterances in the publications. 
% Next, we manually filter out utterances that do not meet our requirements.
% As a result, we obtain $629$ utterances in total, where $249$ are from the sports domain and the rest fall in the urban domain.

% \subsubsection{Results}
% The task distribution of each domain is shown in Figure~\ref{fig:paper_task}. 
% The y-axis presents task categories, while the x-axis means the proportion of tasks in each field.
% We observe that some tasks are dominant in both domains, such as \textit{Cluster}, and \textit{Correlation}. 
% Since the number of entities, \eg, candidate solutions or tactics, is large in both domains.
% Clustering is usually applied to group similar entities and provide an overview of the entire dataset.
% For example, in a billboard placement project in the urban domain, analysts ask, \textit{``How many groups of candidate solutions exist?''}
% Similarly, analysts in the sports domain often seek to understand \textit{``What are the frequent patterns of tactics?''}
% In the sports domain, \textit{Correlation} ranks first among all tasks. 
% By scrutinizing the paper, we find that analysts often need to understand the potential effect of a particular adjustment in tactics.
% They may ask questions such as, \textit{``How does a tactical adjustment influence the strokes and tactics''}, and \textit{``What is the effect of a formation change?''}
% An interesting finding is that publications in the urban domain constitute a larger portion of \textit{Characterize Distribution} tasks ($17.63\%$) compared to the sports domain ($8.03\%$).
% Since the Urban domain usually involves the analysis of spatial-temporal data.
% Analysts may ask questions such as \textit{``How are the target trajectories distributed across the city''}, and \textit{``What is the difference between weekday and weekend?''}



% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=.5\linewidth]{pictures/paper_task.pdf}
%     \caption{Comparison of task analysis between two domains, \ie, sports and urban computing. The x-axis presents the proportion of analytic tasks in each domain.}
%     \label{fig:paper_task}
% \end{figure}


==> src/corpusAnalysis.tex <==
\section{\name{} Characteristics}
In this section, we demonstrate the characteristics of \name{} as compared to other popular datasets through 1) statistical analysis of these corpora and 2) benchmarking of a range of learning-based approaches. 
Based on the potential usage of our corpus, we focus on two fundamental NLP tasks, namely, text classification and paraphrase generation.
% In this section, we demonstrate four applications of \name{}. 
% The first set of experiments exploits the characteristics of our corpus in the text classification task.
% The second experiment underlines the advantages of having paraphrases for each expert query.
% The first two experiments shows how \name{} can serve as a benchmark for text classification and paraphrase generation, respectively.
% The third experiment explores a potential usage of \name{} to support natural language interfaces,
% whereas the last experiment outlines how our corpus can be generalized to analyze design tasks described in academic publications.
% two applications, \ie, sports data analysis and urban computing.

\subsection{Text Classification}
\label{subsec:textclassification}

% \begin{table}
%     \centering
%     \begin{tabular}{r|c|c|c|c}
%     \toprule
%         \textbf{Dataset} & \textbf{CNN} & \textbf{C-LSTM} & \textbf{C-CNN} & \textbf{Ad-RNN} \\ \midrule
%         % Quda\_random &  94.18  &  94.31  &  94.36  &  95.31   \\ \midrule
%         Quda\_expert &  66.12  &  64.89  &  62.68  &  65.90   \\ \midrule
%         % Quda\_aug\_random&  88.51  &  89.43  &  88.41  &  89.95   \\ \midrule
%         Quda\_aug\_expert&  67.31  &  69.20  &  66.17  &  69.47  \\ \midrule
%         TREC &  77.20  &  77.42  &  77.64  &  78.04   \\ \midrule
%         SST &  38.85  &  41.34  &  40.06  &  42.65   \\ \bottomrule
%     \end{tabular}
%     \vspace{1mm}
%     \caption{The performance of four well-performed text classification models on four datasets. We report precision scores in the experiment.}
%     \label{tab:classify_result}
% \end{table}

\subsubsection{Statistical Analysis}
\name{} contains $10$ categories, $14,035$ sentences with $12.62$ average sentence length. 
Compare to some well-known datasets designed for benchmarking deep text classification models, i.e., TREC ($5,952$ sentences, six categories) and SST\cite{Socher2013} ($11,748$ sentences, five categories), \name{} not only has a comparable scale but offers a new sub-domain that focuses on query intention classification.  
These unique properties make \name{} the largest corpus in the domain of visual data analytics to date.


% We compare our corpus ($10$ categories, \siwei{$14,035$} sentences with \siwei{$10.34$} average sentence length) to two corpora containing multiple category labels (greater than 2) for text classification, \ie, TREC and SST.
% TREC contains  falling into  six categories. The average sentence length is about \siwei{$9.35$}. 
% SST includes five categories for . The average sentence length is \siwei{$12.35$}.
% % These corpora vary significantly in size, number of categories, and average sentence length.
% \name{} exceeds TREC and SST in the number of categories, the number of sentences, and the average sentence length, which provides new training and evaluation standards for text classification models.
% % Though AG's News contains more samples, 
% \name{} is the largest corpus in the domain of visual data analytics to date. 
% \siwei{experiment with AG's News}.


\subsubsection{Benchmarking}
Assigning a task label to a query is critical in  V-NLIs.
Therefore, we conduct an experiment to evaluate how text classification models perform on our corpus, and reveal the characteristics of our corpus with different experiment settings.

\textbf{Models:}
We conduct our experiment with four well-known text classification models as baselines. 
The first is a convolutional neural network \textit{CNN}~\cite{Kim2014} built on top of pre-trained word vectors for sentence classification.
The second model, \textit{C-LSTM}~\cite{Zhou2015}, utilizes the strength of CNN and long short-term memory recurrent neural networks (LSTM).
The third is the \textit{C-CNN} model that adds a recurrent connection to the convolutional layer\cite{Shin2018}.
Lastly, we employ \textit{Ad-RNN}~\cite{Miyato2016}, which uses adversarial and virtual adversarial training to improve the RNN model.
We use the default parameter settings for all models.

\textbf{Dataset:} 
We have prepared two corpora in this experiment.
Different data splits (train and test) may affect the performance of models.
We split the dataset by experts. That is, $20$ experts are split into train and test sets (\name{}\_expert).
All queries created by the same experts and their paraphrases are in the same set.
% We split the dataset using two approaches to reveal the characteristics of \name{} and the generalizability of models.
% (1) \textit{Split randomly}. Examples are randomly split into train and test sets (\name{}\_random). 
% Queries referring to the same data table and expert sentence can appear in both train and test.
% (2) \textit{Split by experts}. $20$ experts are equally split into train and test sets (\name{}\_expert). 
% All queries created by the same expert and their paraphrases are in the same set.
We observed that high-frequency words that appeared in the \name{} queries may have strong correlations with the contents in the data tables, that is, these words or phrases are values in data tables or synonyms of column names.  
These correlations may introduce biases and make the model ignoring the real intentions of the queries, and therefore hurting the model generalization.
Inspired by prior work \cite{Zhang2015}, we further employ a data augmentation technique on \name{} that replaces words or phrases with their synonyms.
To be specific, we derive a list of $210$ high-frequent words after stop-words removal. 
Then we manually categorize these words into five groups, \ie, Place, Person, Time, Date, and Others.
Next, for each group, we compile a set of alternative words from WordNet\cite{Fellbaum2000}, and replace high-frequent words with the alternatives randomly.
% and randomly replace high-frequent data-related words with a pool of alternatives. 
% Technique details can be found in \siwei{supplimentary materials}.
Finally, we split the augmented corpus by experts and obtain \name{}\_aug\_expert.
% Further, we use the two splitting strategies and obtain \name{}\_aug\_expert and \name{}\_aug\_random, respectively.
% In addition, we evaluate models on TREC-6~\cite{Voorhees1999} and SST\cite{Socher2013}, which are to commonly used for benchmarking.
To reduce bias in data split, we report the average F1 scores of 10-fold cross-validation to estimate the performance of models on these corpora.
% (2) \textit{Split by expert sentences}. $920$ expert sentences are randomly split into $10$ sets. All associated paraphrases are in the same set.
% (3) \textit{Split by data tables}. $35$ data tables are split into $10$ sets. 
% All queries referring to the same data table are in the same set.


\begin{figure}[tb]
    \centering
    \includegraphics[width=.5\linewidth]{pictures/classify_result.pdf}
    \caption{The performance of four well-known text classification baseline models on \name{}\_expert and \name\_aug\_expert in terms of F1 score.}
    \label{fig:classify_result}
\end{figure}


\textbf{Results:}
Figure~\ref{fig:classify_result} shows the performance of four baseline models on \name{} corpora in terms of precision. Compare to the SOTA precision of the other datasets for text classification at a similar scale (e.g., TREC-$98.07\%$\cite{Cer2018}), the numbers in Figure~\ref{fig:classify_result} indicate that classifying the \name{} queries is challenging, and this leaves room for developing new methods that specifically designed for this task. 
As shown in Figure~\ref{fig:classify_result}, on average, the augmented corpus (i.e., \name{}\_aug\_expert) increases the precision for about $3.14\%$. This proves that the data augmentation we introduced in this paper is useful for model generalization.

% Table~\ref{tab:classify_result} shows the precision of four models on different corpora.
% Models trained on \name{} have worse performance than TREC, indicating that our corpus is another challenging dataset for text classification.
% On average, \name{}\_expert achieves $64.9\%$ precision while \name{}\_aug\_expert achieves $68.04\%$.
% The augmented corpus increases the precision of models for about $3.14\%$.
% We infer that data tables have strong influence on the model performance.
% By investigating the process of data augmentation, we observe that high-frequently appeared words are mostly data-related.
% That is, these words or phrases are values in data tables or synonyms of column names.
% Such data augmentation decreases the influence of data tables and is useful for controlling generalization error for deep learning models.
% By observing the first and second rows of Table~\ref{tab:classify_result}, we find that randomly split \name{} results in significantly better performance compared to \textit{Split by experts}. 
% On average, four models improve for about $29.64\%$ between two data splits.
% With data augmentation, the influence of data tables decreases and 
% Each experts create sentences with limited data tables (2$\sim$3 in our experiment). 
% Hence, some data values or terms are repeated appeared in the queries.
% Further, paraphrases containing almost the same data values might exaggerate the influence of data tables.
% As a result, models trained on training set 

% As a result, the generalizability to other datasets might be decreased \siwei{interprete the results by Prof. Tang}.



% We infer two reasons for this observation.
% First, text classification for multiple categories is challenging.
% Models achieve the precision of $77.58\%$ and $40.73\%$ on TREC and SST, respectively.
% Therefore, the precision of $64.9\%$ is reasonable for sentences created by different experts with various data tables.
% Second, experts create sentences with limited data tables (2$\sim$3 in our experiment). 
% Hence, similar data values may appear frequently in sentences created by one expert.
% Further, paraphrases containing almost the same data values might exaggerate the influence of data tables.
% High precision for random split indicates that models trained on our corpus might overfit for data tables used in our experiment.
% As a result, the generalizability to other datasets might be decreased \siwei{interprete the results by Prof. Tang}.

% To lower the influence of data tables, we train and test the same models on \name{}\_aug. 
% As observed in Table~\ref{tab:classify_result}, models perform better on \name{}\_aug\_random ($89.08\%$ on average) than \name{}\_aug\_expert ($68.04\%$ on average). 
% Compared to \name{}, the precision for \textit{Split randomly} decreases while it increases for \textit{Split by experts}. 
% It is inferred that, with data augmentation, we lower the influence of data tables, and improve the generalizability of models trained using our corpus.
% We also note that the difference of precision between two data splits ($89.08\%-68.04\%=21.04\%$) decreases compared to that of \name{}, which is $29.64\%$.
% However, the difference remains significant.
% Though we have reduced the influence of data tables, sentences created by the same experts, associated with paraphrases, may have latent characteristics that are influential on task classification.
% Further research is required to provide explainability for latent characteristics on these corpora.


% \subsection{Paraphrase Generation}
% Paraphrase generation is important in NLP and can be beneficial for a wide range of downstream applications, such as question answering, semantic parsing, information retrieval, text summarization, among others~\cite{Li2018}.
% Each expert query is accompanied by $14$ paraphrases, and thus, our corpus can serve as a benchmark for paraphrase identification, extraction, generation, etc.
% We explore the properties of \name{} in the context of paraphrase generation.

% \subsubsection{Statistical Analysis}
% Table~\ref{tab:para_stat} shows the statistical information of \name{} in comparison with other paraphrasing corpora. 
% The Quora dataset\cite{quora} is a collection of question paraphrases composed of over $148,130$ pairs of duplicate questions.
% It has about $148,532$ unique sentences.
% We follow the experimental protocols mentioned by Patro \etal~\cite{Patro2018} to sample $50$K (Quora-$50$K) and $100K$ (Quora-$100$K) as training sets and use the rest of the $10$K and $30$K as test sets, respectively.
% The Twitter dataset\cite{Lan2017}, which is widely used for paraphrasing research, consists of a large amount of human-annotated sentence pairs, which are collected from Twitter by linking tweets through shared URLs.
% This dataset is growing continuously and has $114,025$ pairs of paraphrases ($88,938$ unique sentences) after a one-year collection (from 2016.10 to 2017.10)~\cite{Socher2013}.
% We sample $100$K randomly as a training set (Twitter-$100$K) and $15$K as the testing set.
% % By following Gupta \etal's work, we sample 100K pairs and create the Twitter-100K dataset.
% We construct paraphrasing datasets from \name{} using two settings.
% First, we allow sentence repeat using permutations (\name{}-78K). 
% For example, given $15$ sentences ($1$ expert sentence + $14$ paraphrases) with the same meaning, we construct $\binom{2}{15}=105$ pairs.
% As a result, each sentence will appear in multiple paraphrase pairs, and we have $78,939$ pairs consisting of $11,102$ unique sentences.
% Second, we avoid sentence repeat by selecting $7$ pairs randomly from $15$ sentences, which results $5,365$ pairs ($10,730$ unique sentences) in total (\name{}-5K).
% For the \name{}-5K and \name{}-78K datasets, we split the train (90\%) and test (10\%) randomly as shown in Table~\ref{tab:para_stat}.


% % Compared to the Twitter dataset, \name{}-5K and \name{}-78K are not competitive in scale in terms of number of pairs and unique sentences because Quora or Twitter-based utterances are mainly for general purpose and cover a large range of topics.
% % However, \name{}-5K and \name{}-78K are tailed for data analytics, and queries in \name{} reflect how analysts may ask questions on the data.
% % \name{} differs from the other paraphrasing corpora (e.g., Twitter dataset) from both vocabulary space and design purposes. 
% % Therefore, it provides a new data source with new problems that complementary to all existing paraphrasing corpora.

% Compared to the dataset like Quora or Twitter, \name{} differs from them for both vocabulary space and design principles. 
% \name{}-5K and \name{}-78K are tailed for data analytics, and the queries in \name{} reflect how analysts may ask questions on the data. 
% On the other hand, utterances in Quora or Twitter datasets are mainly for general purpose and therefore cover a large range of casual topics. 
% In summary, although \name{}-5K and \name{}-78K are not competitive to Quora or Twitter dataset in terms of the number of pairs and unique sentences, it provides a new data source with new problems that complementary to all existing paraphrasing corpora.

% \subsubsection{Benchmarking}
% We first define the task of paraphrase generation, then introduce the setup of the experiment. 
% Finally, we present the benchmarking results to provide deep insights into our corpus in comparison to others.

% \textbf{Task Definition:}
% We follow the description in Patro \etal's work~\cite{Patro2018} to introduce the task of paraphrase generation.
% Given an original sentence and a reference sentence $(x^o, x^r)$ with almost the same meaning, we need to generate another sentence $y$ so that the distance between $y$ and the reference $x^r$ is minimal.
% The training data $S$ consist of $M$ pairs of paraphrases $S=\{(x^o_i, x^r_i)\}^M_{i=1}$, where $x^o_i$ and $x^r_i$ are paraphrases of each other. 

% \begin{table}
%     \centering
%     \begin{tabular}{r|c|c|c|c}
%         \toprule
%         \textbf{Dataset} & \textbf{\# Pairs} & \textbf{\#  Sentences} & \textbf{Train} & \textbf{Test} \\ \midrule
%         Quda-5k & 5,365 & 10,730 & 5,365 & 684 \\ \midrule
%         Quda-78k & 78,939 & 11,102 & 78,939 & 10,302 \\ \midrule 
%         Quora-50k & 50,000 & 66,621 & 50,000 & 10,000 \\ \midrule
%         Quora-100k & 100,000 & 112,397 & 100,000 & 30,000 \\ \midrule
%         Twitter-100k & 100,000 & 31,465 & 100,000 & 15,000 \\
%         \bottomrule
%     \end{tabular}
%     \vspace{1mm}
%     \caption{Statistical comparison between five paraphrasing datasets.}
%     \label{tab:para_stat}
% \end{table}

% \textbf{Models:}
% We choose three representative techniques for paraphrase generation.
% The first model (\textit{EDLPS}) proposes a pairwise discriminator based encoder-decoder for paraphrase generation.  
% Encoder, decoder, and discriminator are built upon LSTM~\cite{Patro2018}.
% Second, we choose \textit{VAE-SVG}, which combines deep generative models (VAE) with  sequence-to-sequence models (LSTM).
% This model can generate multiple paraphrases for a given sentence~\cite{Gupta2018}.
% The third model (\textit{DiPS}) can generate paraphrases similar in semantics yet diverse in structure. 
% The model is based on a basic Seq2Seq framework and features in monotone sub-modular function maximization~\cite{Kumar2019}.
% We use the same parameter setting on all datasets for each model.

% \textbf{Evaluation Metrics:}
% The evaluation metrics include METEOR~\cite{Lavie2007}, BLEU~\cite{Papineni2002}, and TER~\cite{Snover2006}.
% Though these metrics were used originally for machine translation, prior research has shown that they correlate with human judgments in terms of evaluating the quality of the generated paraphrases~\cite{Wubben2010}.
% BLEU score considers the modified n-gram precisions and poses penalty for paraphrases that are too short or too long.
% We use the unigram precisions to present the results.
% The higher the BLEU score is, the better the generated paraphrases are in quality.
% METEOR calculates word mapping, unigram precision and recall between the generated paraphrase and the reference sentence.
% A higher METEOR score reflects better paraphrasing quality.
% TER stands for Translation Edit Rate, which measures how much effort humans would have to perform to change a generated paraphrase to the reference.
% Lower TER scores mean better quality.


% \textbf{Results:}
% Table~\ref{tab:para_result} shows the performance of three models using four datasets under three metrics.
% Generally, models do not perform well on \name{}-5K compared to other datasets.
% All models result in lower BLEU score, lower METEOR score, and high TER for \name{}-5K and \name{}-78K. 
% Given the same experimental settings, the performance of the models highly relates to the volume of training sets.
% An interesting observation is that models perform better on Quora-$50$K than \name{}-78K, albeit Quora-$50$K is larger in scale than \name{}-78K.
% That is probably because the number of unique sentences in \name{}-78K is six times smaller than those in Quora-$50$K. 

% \begin{table}
%     \centering
%     \begin{tabular}{r|c|c|c|c}
%     \toprule
%         \textbf{Dataset} & \textbf{Model} & \textbf{BLEU} & \textbf{METEOR} & \textbf{TER} \\ \midrule
%         \multirow{3}{*}{Quda-5k} & EDLPS & 16.1 & 5.2 & 107.6 \\ \cmidrule{2-5}
%          & VAE-SVG & 28.0 & 11.7 & 89.0 \\ \cmidrule{2-5}
%          & DiPS & 19.1 & 7.9 & 92.3 \\ \midrule
%         \multirow{3}{*}{Quda-78k} & EDLPS & 21.1 & 8.2 & 98.6 \\ \cmidrule{2-5}
%          & VAE-SVG & 26.6 & 12.5 & 88.6 \\ \cmidrule{2-5}
%          & DiPS & 24.1 & 9.5 & 94.8 \\ \midrule
%         \multirow{3}{*}{Quora-50k} & EDLPS & 29.6 & 14.5 & 87.9 \\ \cmidrule{2-5}
%          & VAE-SVG & 40.8 & 21.6 & 74.4 \\ \cmidrule{2-5}
%          & DiPS & 44.8 & 25.1 & 63.9 \\ \midrule
%         \multirow{3}{*}{Quora-100k} & EDLPS & 37.4 & 19.9 & 76.9 \\ \cmidrule{2-5}
%          & VAE-SVG & 42.3 & 23.0 & 70.2 \\ \cmidrule{2-5}
%          & DiPS & 45.9 & 25.9 & 63.1 \\
%         % \multirow{3}{*}{Twitter-100k} & EDLPS & 32.3 & 17.2 & 83.3 \\ \cmidrule{2-5}
%         %  & VAE-SVG & 48.7 & 26.5 & 66.7 \\ \cmidrule{2-5}
%         %  & DiPS & 52.3 & 29.3 & 61.4 \\ \midrule
%          \bottomrule
%     \end{tabular}
%     \vspace{1mm}
%     \caption{The performance of three paraphrase generation models on four datasets measured using BLEU, METEOR, and TER. }
%     \label{tab:para_result}
% \end{table}



